Hybridization of interval methods and evolutionary algorithms for solving difficult optimization problems

Reliable global optimization is dedicated to finding a global minimum in the presence of rounding errors. The only approaches for achieving a numerical proof of global optimality are interval branch and bound methods that interleave branching of the search-space and pruning of the subdomains that cannot contain an optimal solution. It is of the utmost importance: i) to compute sharp enclosures of the objective function and the constraints on a given subdomain; ii) to find a good approximation (an upper bound) of the global minimum. State-of-the-art solvers are generally integrative methods, that is they embed local optimization algorithms to compute a good upper bound of the global minimum over each subspace. In this document, we propose a cooperative framework in which interval methods cooperate with evolutionary algorithms. The latter are stochastic algorithms in which a population of candidate solutions iteratively evolves in the search-space to reach satisfactory solutions. Evolutionary algorithms, endowed with operators that help individuals escape from local minima, are particularly suited for difficult problems on which traditional methods struggle to converge. Within our cooperative solver Charibde, the evolutionary algorithm and the interval-based algorithm run in parallel and exchange bounds, solutions and search-space via message passing. A novel strategy prevents premature convergence toward local minima. A comparison of Charibde with state-of-the-art solvers (GlobSol, IBBA, Ibex) on a benchmark of difficult problems shows that Charibde converges faster by an order of magnitude. New optimality results are provided for five multimodal problems, for which few solutions were available in the literature. Finally, we provide the first numerical proof of optimality for the open Lennard-Jones cluster problem with five atoms.

==> chapters/conflicts.tex <==
\chapter{Contribution to aircraft conflict resolution}
\label{chap:conflits}

\minitoc

La résolution de conflits aériens, modélisée sous la forme d'un problème d'optimisation sous
contraintes, est un problème fortement combinatoire et très contraint. Il consiste à générer des
trajectoires les plus proches possibles des trajectoires initiales, tout en respectant la
séparation entre avions à tout instant.

Les différentes approches de résolution de conflits sont introduites dans la section
\ref{sec:conflits}. Dans la section \ref{sec:conflits-ae}, nous proposons une approche en changement
de cap paramétrée par des variables continues et résolue par des algorithms à population. Nous
adoptons dans la section \ref{sec:conflits-charibde} un modèle sous contraintes universellement
quantifiées que nous résolvons à l'optimalité avec des méthodes d'intervalles.

\section{Aircraft conflicts}
\label{sec:conflits}
Le trafic aérien est organisé en réseaux de routes aériennes, constituées de segments convergeant
vers des points de virages ou waypoints (Figure \ref{fig:carte-aero}). Parfois, des équipements
radio-électriques sont placés au sol en ces points pour permettre aux avions de se situer à l'aide
d'équipements de radionavigation à bord.

\begin{figure}[htb]
\centering
\includegraphics[width=0.8\columnwidth]{figures/conflits/carte.png}
\caption{Carte aéronautique des routes aériennes}
\label{fig:carte-aero}
\end{figure}

\subsection{Separation}
Le contrôle en phase de croisière (ou en route) consiste à gérer la progression des avions en
dehors des zones proches des aéroports. L'objectif principal du service de contrôle au sol est
d'empêcher les collisions entre avions en maintenant à tout instant une séparation des trajectoires
d'au moins 5 milles nautiques (9.3km) sur le plan horizontal et 1000 pieds (305m) verticalement
(Figure \ref{fig:espace-separation}).

\begin{figure}[htb]
\centering
\includegraphics[width=0.5\columnwidth]{figures/conflits/bounding_volume}
\caption{Espace de séparation pour la phase de croisière}
\label{fig:espace-separation}
\end{figure}

Un \textit{conflit} est une perte de séparation entre les prévisions de trajectoires. La résolution
de conflits entre trajectoires d'avions consiste à man\oe uvrer les appareils pour garantir leur
séparation à tout instant. Différents types de man\oe uvres sont généralement considérés: les
allocations de niveaux de vol, la résolution en vitesse et les évitements latéraux.
L'\textit{allocation de niveaux de vol} concerne les changements d'altitude, à
raison d'un niveau de vol disponible tous les 100 pieds (30m). La \textit{résolution en vitesse} est
une modification de la vitesse de l'avion en tenant compte de contraintes de bornes sur
l'accélération. L'\textit{évitement latéral} est un changement de cap dans le plan horizontal.

\subsection{Approaches for conflict resolution}
Deux types d'approches existent pour la résolution de conflits: les approches \textit{autonomes}
(ou distribuées) dans lesquelles chaque avion est équipé d'un système de contrôle embarqué et n'a
qu'une visibilité limitée des appareils qui l'entourent, et les approches \textit{centralisées}
dans lesquelles les contrôleurs aériens au sol ont un aperçu global du trafic.

Les approches autonomes ont été conçues dans les années 1990 dans le cadre de la méthode de
contrôle aérien Free Flight. Elles laissent la liberté au pilote de s'affranchir en partie des
restrictions de vol, et de sélectionner des trajectoires en temps réel. \cite{Zeghal1998} exploite
des champs de forces: la cohérence des mouvements de plusieurs objets mobiles repose sur la
définition de force glissante entre deux objets. Il n'existe néanmoins aucune garantie d'optimalité
au-delà de deux avions. FACES~\cite{Durand2000Faces} est un solveur de conflits embarqué dédié à
l'espace aérien de Free Flight, dans lequel la coordination entre appareils est garantie par une
stratégie d'allocation de jeton. Les conflits sont résolus par un algorithm $A^*$ après que les
vols ont été classés par niveau de priorité. Cette approche a fait l'objet de tests intensifs
impliquant un petit nombre d'avions dans le simulateur CATS~\cite{Cats1997} ; seule l'optimalité
locale
est assurée. Un algorithm de détection et d'analyse des conflits potentiels en phase de
croisière~\cite{Isaacson1997Design} génère l'ensemble des conflits futurs probables, et assiste le
contrôleur dans la tâche de résolution de son secteur. Les conflits sont détectés par comparaison
des trajectoires à des instants consécutifs proches.

Les seules approches centralisées permettant de résoudre efficacement des conflits impliquant plus
d'une vingtaine d'avions en recherchant un optimum global, sont la programmation linéaire mixte
\cite{Pallottino2002,Brisset2010} et les \gls{EA} \cite{Durand1996,Delahaye2010,Vanaret2012}.
Dans \cite{Pallottino2002}, les hypothèses sur la vitesse des avions sont fortes et peu réalistes
dans le cadre d'une utilisation opérationnelle: vitesses constantes pour des résolutions par
évitement latéral, ou changements de vitesses instantanés pour des résolutions en vitesse. Dans
\cite{Durand1996}, un \gls{GA} fait évoluer une population d'individus encodant des man\oe uvres de
déviations latérales pour les avions initialement en conflit. La modélisation proposée s'appuie sur
des variables discrétisées (temps de début et de fin de man\oe uvres, angles de déviation). Les
hypothèses relativement réalistes, permettant notamment la prise en compte d'incertitudes sur les
vitesses, donnent des résultats très convaincants. Dans \cite{Delahaye2010}, les déviations
latérales sont approximées par des B-splines. Les changements de cap continus rendent l'approche
inexploitable par les systèmes de gestion de vol ou \gls{FMS}. Dans \cite{Vanaret2012}, des man\oe
uvres rectilignes par morceaux, paramétrées par des variables continues et optimisées par des
\gls{EA}, fournissent une séquence de waypoints directement exploitable par les \gls{FMS}.

\subsection{Maneuver model}
\begin{figure}[htbp]
\centering
\def\svgwidth{0.6\columnwidth}
\input{figures/conflits/point_tournant.pdf_tex}
\caption{Point tournant}
\label{fig:point-tournant}
\end{figure}

Each maneuver is parameterized by a triplet $(d, \alpha, l)$, et suit une
trajectoire constituée d'un segment rectiligne écartant l'avion de sa trajectoire initiale, suivi
a return segment (see Figure \ref{fig:point-tournant}). 

La man\oe uvre par évitement latéral d'une trajectoire $i$ est modélisée par un point tournant
(Figure \ref{fig:point-tournant}). Elle est caractérisée par un triplet de réels $(d_i,
\alpha_i, l_i)$: l'avion s'écarte de sa trajectoire initiale après une distance $d_i$, avec un
angle de déviation $\alpha_i$. Après avoir parcouru le segment de déviation de longueur $l_i$,
l'avion revient à sa trajectoire initiale avec un angle $-2\alpha_i$. Une configuration à $N$
avions est donc représentable par un vecteur de $n = 3N$ variables continues.

\section{Centralized approach using evolutionary algorithms}
\label{sec:conflits-ae}
Nous avons introduit dans \cite{Vanaret2012} un benchmark de problèmes de résolution de conflits,
sur lequel nous avons comparé les performances de trois algorithms à population. La résolution
de conflits est modélisée par un problème d'optimisation sous contraintes: le but de la résolution
est de générer des trajectoires les plus proches possibles des trajectoires initiales, tout en
respectant la séparation entre avions à tout instant. Nous adoptons une approche "boîte noire", dans
la mesure où l'évaluation des contraintes de séparation nécessite de simuler les
trajectoires grâce à un petit simulateur de trafic.

Notre modèle, basé sur des man\oe uvres latérales, est identique à celui de \cite{Pallottino2002}.
Il pourrait aisément être étendu à des man\oe uvres verticales et en vitesse. Contrairement à
\cite{Durand1996}, le début de man\oe uvre, l'angle et la longueur de déviation sont des variables
continues. Nous comparons sur le benchmark proposé trois algorithms à
population manipulant des variables continues: un \gls{GA} avec un encodage réel, une \gls{PSO} et
une \gls{DE}. Les résultats obtenus mettent en lumière la supériorité de certains algorithms sur le
problème de résolution de conflits.

\subsection{Constrained optimization problem}

\subsubsection{Separation constraints}
Notons $\vec{p_i}(t)$ et $\vec{p_j}(t)$ les positions de deux avions $i$ et $j$ à un instant $t$.
La contrainte de séparation entre les deux avions est donnée par:
\begin{equation}
S^2 \le \|\vec{p_i}(t) - \vec{p_j}(t)\|_2^2, \quad \forall t \in [0, T_f]
\label{eq:contrainte-separation}
\end{equation}
où $[0, T_f]$ est l'intervalle de temps considéré et $\|\cdot\|_2$ est la norme euclidienne. La
Figure \ref{fig:norme-separation} illustre les zones de séparation de cinq avions, représentées
dans le plan horizontal par des cercles de diamètre $S$, centrés sur les appareils, qui ne doivent
s'intersecter à aucun moment. 
\begin{figure}[htbp]
\centering
\includegraphics[width=0.5\columnwidth]{figures/conflits/separations}
\caption{Zones de séparation}
\label{fig:norme-separation}
\end{figure}

\subsubsection{Objective function}
Afin de réduire la déviation induite par la man\oe uvre, l'angle et la longueur du segment de
déviation doivent être les plus faibles possibles. En revanche, le début de la man\oe uvre doit
être repoussé au plus tard, de sorte que les man\oe uvres prématurées futures soient réduites
ou évitées (en raison de la diminution de l'incertitude sur la position des avions). En notant
$\bm{x} = (d_1, \alpha_1, l_1, \ldots, d_N, \alpha_N, l_N)$ les variables de décision, la fonction
objectif s'exprime comme
une somme de carrés:
\begin{equation}
f(\bm{x}) = \sum_{i=1}^N \left( (1-\frac{d_i}{\overline{d_i}})^2 +
(\frac{\alpha_i}{\overline{\alpha_i}})^2 + (\frac{l_i}{\overline{l_i}})^2 \right)
\end{equation}

Le problème d'optimisation sous contraintes modélisant le problème de résolution de conflits
aériens est alors le suivant:
\begin{equation}
\label{eq:resolution-conflits}
\begin{aligned}
\min_{\bm{x}} \quad & \sum_{i=1}^N \left( (1-\frac{d_i}{\overline{d_i}})^2 +
(\frac{\alpha_i}{\overline{\alpha_i}})^2 + (\frac{l_i}{\overline{l_i}})^2 \right) \\
\text{s.t.} \quad	& d_i \in [\underline{d_i}, \overline{d_i}] \\
					& \alpha_i \in [\underline{\alpha_i}, \overline{\alpha_i}] \\
					& l_i \in [\underline{l_i}, \overline{l_i}] \\
					& \forall i < j, \quad S^2 \le \|\vec{p_i}(t) - \vec{p_j}(t)\|^2, \quad \forall t \in [0, T_f]
\end{aligned}
\end{equation}

\subsection{Traffic simulator}
Pour pallier le manque de résultats dans la littérature concernant la résolution de conflits
aériens, nous avons proposé une bibliothèque OCaml encapsulant un petit simulateur de trafic
aérien. Une fonction $\mathit{conflits}$ calcule la violation des contraintes de séparation pour un
vecteur de déviations latérales $\bm{x}$ donné. Un conflit est ici défini par un intervalle compact
de temps pendant lequel la contrainte de séparation entre les avions $i$ et $j$ (équation
\ref{eq:contrainte-separation}) est violée. Puisque plusieurs conflits peuvent avoir lieu entre deux
avions, le terme $C_{i,j}$ de la matrice $C$ obtenue en invoquant $\mathit{conflits}(\bm{x})$
représente une
liste des durées des conflits entre les avions $i$ et $j$. La matrice $C$ rend donc directement
accessibles le nombre et la durée des conflits. Lorsque les segments de trajectoires sont linéaires,
les conflits peuvent être détectés en résolvant une équation du second degré (à vitesses constantes)
ou une équation du quatrième degré (à accélérations constantes).

Le simulateur est doté de nouvelles fonctionnalités en comparaison de précédents simulateurs,
tels que CATS/OPAS~\cite{Cats1997}: les actions possibles (accélérer, suivre une route, etc.)
sont modélisées comme les arêtes d'un graphe orienté acyclique (DAG), dont les n\oe uds
déclenchent des événements (par exemple, capture de vitesse ou de waypoint). Les trajectoires
sont prédites avec un pas de temps par défaut constant $\delta{t}$ et les conflits sont
détectés deux à deux en considérant les distances entre avions. Néanmoins, un pas de temps plus
faible est considéré lorsqu'un événement est déclenché entre le temps courant $t$ et le temps
suivant $t + \delta{t}$ dans la boucle de simulation. Ceci permet de simuler des déviations
latérales dont les variables $(d_i, \alpha_i, l_i)$ sont continues (plutôt que de discrétiser
leurs domaines~\cite{Durand1996}) et d'utiliser des méthodes d'optimisation continue.

Les plans de vol des avions et leurs états initiaux sont chargés depuis un fichier XML, ainsi que
les paramètres de simulation et les domaines des variables paramétrant les déviations de
trajectoires. Les fichiers XML standardisés peuvent alors être mis à disposition de la
communauté de trafic aérien.

\subsection{Test problems}
Nous considérons deux configurations de test à $N$ avions: une configuration initiale $C_N$ en
cercle (Figure \ref{fig:conflits-cercle}, les dimensions sont en milles nautiques) et une
configuration $B_N$ en cercle bruité (Figure \ref{fig:conflits-rand}):

\begin{enumerate}[label=\alph*)]
\item Configuration initiale $C_N$ en cercle:
les avions sont arrangés régulièrement autour d'un cercle, et leurs trajectoires convergent
simultanément vers
le centre du cercle. Deux solutions optimales existent: tous les avions tournent soit à droite,
soit à gauche. Ces configurations sont appelées "ronds-points".

\begin{figure}[htb]
\centering
\includegraphics[width=0.7\columnwidth]{expes/conflits/benchmark/cercle10}
\caption{Configuration initiale $C_{10}$ en cercle}
\label{fig:conflits-cercle}
\end{figure}

Il s'agit d'un problème très contraint. Pour s'en convaincre, on peut dénombrer le nombre de
situations sans conflits parmi un million de configurations de man\oe uvres à $N$ avions générées
aléatoirement: 
pour $N = 5$, seules 497 situations satisfont les contraintes de séparation. Pour $N > 8$, aucune
des situations générées n'est sans conflit;

\item Configuration initiale $B_N$ en cercle bruité:
bien que très combinatoire, $C_N$ reste un problème symétrique. Afin de complexifier les
comportements des avions, nous introduisons une deuxième configuration initiale de test dans
laquelle les avions sont à l'identique disposés sur un cercle, et leurs caps par rapport au
diamètre du cercle sont tirés aléatoirement dans $[-\frac{\pi}{6}, \frac{\pi}{6}]$.
Le point final de la trajectoire appartient également au cercle.

\begin{figure}[htb]
\centering
\includegraphics[width=0.7\columnwidth]{expes/conflits/benchmark/rand10}
\caption{Configuration initiale $B_{10}$ en cercle bruité}
\label{fig:conflits-rand}
\end{figure}

\end{enumerate}

\subsection{Experimental results}
Nous comparons les résolutions obtenues par trois algorithms à population (un \gls{GA}, une
\gls{PSO} et une \gls{DE}) sur les deux configurations $C_N$ et $B_N$ avec une séparation de $S =
5$ NM. Le nombre maximum d'évaluations de la fonction objectif est fixé à 120000.

Les Figures \ref{fig:conflits-c25} à \ref{fig:conflits-b50} (en échelle logarithmique sur l'axe
des abscisses) décrivent, pour diverses instances du problème, l'évolution du meilleur individu
en fonction du nombre d'évaluations de la fonction objectif. Les courbes sont séparées en deux
parties: les courbes du haut représentent la durée totale de conflits restants entre les $N$
avions, et les courbes du bas affichent l'évaluation du meilleur individu une fois les conflits
résolus. La Figure \ref{fig:conflits-c25} montre que les trois algorithms à population utilisés
produisent des solutions relativement proches en terme de valeur objectif pour le problème
$C_{25}$ (40.2 pour l\gls{DE}, 46.7 pour l'\gls{GA} et 49.1 pour l'\gls{PSO}), bien que le nombre
d'évaluations nécessaires pour résoudre les conflits varie grandement (10800 pour % d'un rapport 7
l'\gls{DE}, 43200 pour l'\gls{GA} et 68250 pour l'\gls{PSO}). La solution du problème obtenue par
une \gls{DE}, proche de la configuration optimale en rond-point dans laquelle tous les avions
tournent à droite, est présentée en Figure \ref{fig:solution-c25}.

\begin{figure}[htb]
\centering
\includegraphics[width=0.7\columnwidth]{expes/conflits/benchmark/solution25}
\caption{Solution du problème $C_{25}$ par un algorithm à évolution différentielle}
\label{fig:solution-c25}
\end{figure}

Les Figures \ref{fig:conflits-b20} (problème $B_{20}$) et \ref{fig:conflits-b30} (problème
$B_{30}$) suggèrent que l'\gls{PSO} est capable de résoudre les conflits en peu d'itérations sur
les instances les plus petites, mais peine à explorer l'espace de recherche sur les instances plus
importantes et reste piégée dans des minima locaux. En revanche, l'\gls{GA} et l'\gls{DE} semblent
dotés de mécanismes d'exploration efficaces, capables de s'échapper des minima locaux. Ces deux
problèmes donnent un léger avantage à l'\gls{DE}. La Figure
\ref{fig:solution-b20} illustre la meilleure solution trouvée par chacun des algorithms à
population utilisés sur le problème $B_{20}$. On notera que, malgré le faible écart entre les
évaluations de l'\gls{GA} et l'\gls{DE}, leurs solutions apparaissent visuellement différentes.

La tendance s'inverse sur les problèmes $B_{40}$ (Figure \ref{fig:conflits-b40}) et $B_{50}$
(Figure \ref{fig:conflits-b50}) ; bien qu'un peu plus lent pour résoudre les conflits, l'\gls{GA}
obtient une solution finale meilleure que celle atteinte par l'\gls{DE}. Quant à l'\gls{PSO}, les
conflits sont de peu résolus pour le problème $B_{40}$ et non résolus pour le problème $B_{50}$.

\begin{figure}[t!]
	\centering
	\subfloat[Algorithme génétique]{\includegraphics[width=0.41\textwidth]{expes/conflits/benchmark/20ag}}
	\subfloat[Essaim particulaire]{\includegraphics[width=0.41\textwidth]{expes/conflits/benchmark/20pso}} \\
	\subfloat[Evolution différentielle]{\includegraphics[width=0.41\textwidth]{expes/conflits/benchmark/20de}}
	\caption{Solutions du problème $B_{20}$}
	\label{fig:solution-b20}
\end{figure}

% C25
\begin{figure}[t!]
	\centering
	\subfloat[Conflits restants]{\includegraphics[width=0.9\textwidth]
	{expes/conflits/benchmark/comparaison/pb1/25/conflits}} \\
	\subfloat[Valeur objectif]{\includegraphics[width=0.9\textwidth]
	{expes/conflits/benchmark/comparaison/pb1/25/fitness}}
	\caption{Problème $C_{25}$}
	\label{fig:conflits-c25}
\end{figure}

% B20
\begin{figure}[t!]
	\centering
	\subfloat[Conflits restants]{\includegraphics[width=0.9\textwidth]
	{expes/conflits/benchmark/comparaison/pb2/20/conflits}} \\
	\subfloat[Valeur objectif]{\includegraphics[width=0.9\textwidth]
	{expes/conflits/benchmark/comparaison/pb2/20/fitness}}
	\caption{Problème $B_{20}$}
	\label{fig:conflits-b20}
\end{figure}

% B30
\begin{figure}[t!]
	\centering
	\subfloat[Conflits
	restants]{\includegraphics[width=0.9\textwidth]
	{expes/conflits/benchmark/comparaison/pb2/30/conflits}} \\
	\subfloat[Valeur
	objectif]{\includegraphics[width=0.9\textwidth]
	{expes/conflits/benchmark/comparaison/pb2/30/fitness}}
	\caption{Problème $B_{30}$}
	\label{fig:conflits-b30}
\end{figure}

% B40
\begin{figure}[t!]
	\centering
	\subfloat[Conflits
	restants]{\includegraphics[width=0.9\textwidth]
	{expes/conflits/benchmark/comparaison/pb2/40/conflits}} \\
	\subfloat[Valeur
	objectif]{\includegraphics[width=0.9\textwidth]
	{expes/conflits/benchmark/comparaison/pb2/40/fitness}}
	\caption{Problème $B_{40}$}
	\label{fig:conflits-b40}
\end{figure}

% B50
\begin{figure}[t!]
	\centering
	\subfloat[Conflits
	restants]{\includegraphics[width=0.9\textwidth]
	{expes/conflits/benchmark/comparaison/pb2/50/conflits}} \\
	\subfloat[Valeur
	objectif]{\includegraphics[width=0.9\textwidth]
	{expes/conflits/benchmark/comparaison/pb2/50/fitness}}
	\caption{Problème $B_{50}$}
	\label{fig:conflits-b50}
\end{figure}

Le tableau \ref{tab:conflits} compile les évaluations des meilleurs individus sur 20 exécutions
par les trois algorithms à population. La colonne 3 indique le nombre d'exécutions non résolues,
c'est-à-dire où il reste des conflits. Les colonnes 4 à 7 donnent les durées minimum, maximum et
moyenne des conflits restants sur les exécutions non résolues et leur écart type. Les colonnes 8 à
11 donnent le coût minimum, maximum et moyen des exécutions sans conflits et leur écart type. Les
deux premières instances $C_{25}$ et $B_{20}$ sont rapidement résolues par l'\gls{GA}, l'\gls{PSO}
et l'\gls{DE}: ceci suggère que les trois algorithms gèrent bien la combinatoire des problèmes.
Lorsque la taille du problème augmente, l'\gls{PSO} perd rapidement en efficacité, en témoigne le
nombre d'exécutions non résolues. Le nombre d'exécutions résolues par l'\gls{GA} diminue peu sur les
grandes instances, tandis que l'\gls{DE} résout toutes les exécutions.

\begin{landscape}
\begin{table}[t!]
	\caption{Durée moyenne des conflits et valeur objectif moyenne sur 20 exécutions, pour 120000
	évaluations de la fonction objectif}
	\label{tab:conflits}
	\centering
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
	\hline
	& & Non résolues & \multicolumn{4}{c|}{Durée des conflits restants (en s)} &
	\multicolumn{4}{c|}{Valeur objectif des exécutions résolues} \\
	\hline
	& Méthode & (sur 20) & Min & Max & Moy & $\sigma$ & Min & Max & Moy & $\sigma$ \\
	\hline
	$C_{25}$ & AG & 0 & - & - & - & - & 46.7291 & 56.7154 & 49.5578 & 2.2153 \\
	& OEP & 0 & - & - & - & - & 49.1103 & 55.1911 & 51.6155 & 1.3208 \\
	& ED & 0 & - & - & - & - & \textbf{40.1904} & 54.7370 & 44.7435 & 3.9793 \\
	\hline
	$B_{20}$ & AG & 0 & - & - & - & - & 11.1921 & 13.8793 & 12.4216 & 0.9086 \\
	& OEP & 0 & - & - & - & - & 26.2831 & 30.2721 & 28.0791 & 1.2368 \\
	& ED & 0 & - & - & - & - & \textbf{9.9302} & 11.8789 & 10.5836 & 0.5232 \\
	\hline
	$B_{30}$ & AG & 5 & 15 & 30 & 21 & 8.2158 & 28.5927 & 36.6782 & 32.8227 & 2.1727 \\
	& OEP & 6 & 15 & 15 & 15 & 0 & 52.8917 & 58.6254 & 55.6343 & 1.8290 \\
	& ED & \textbf{0} & - & - & - & - & \textbf{25.0167} & 33.5501 & 29.6390 & 2.3471 \\
	\hline
	$B_{40}$ & AG & 3 & 15 & 15 & 15 & 0 & \textbf{33.7887} & 46.0925 & 41.3232 & 3.1890 \\
	& OEP & 12 & 15 & 105 & 37.5 & 28.2441 & 64.6237 & 76.2097 & 70.1448 & 3.6213 \\
	& ED & \textbf{0} & - & - & - & - & 45.5938 & 67.4946 & 55.6706 & 6.2888 \\
	\hline
	$B_{50}$ & AG & 3 & 30 & 75 & 45 & 25.9808 & \textbf{56.4666} & 72.5151 & 63.9583 & 3.4726 \\
	& OEP & 20 & 30 & 180 & 129.75 & 41.9422 & - & - & - & - \\
	& ED & \textbf{0} & - & - & - & - & 73.3092 & 115.5933 & 88.7457 & 13.0205 \\
	\hline
	\end{tabular}
\end{table}
\end{landscape}

\subsection{Conclusion and limits of the model}
La comparaison des trois algorithms à population (\gls{GA}, \gls{PSO}, \gls{DE}) sur le benchmark
esquisse une vue d'ensemble des difficultés spécifiques au problème de résolution de conflits,
modélisé par un problème d'optimisation sous contraintes de séparation. Il s'agit d'un problème
combinatoire, très contraint dans de nombreuses (voire toutes les) dimensions de l'espace de
recherche.
En conséquence, les méthodes d'optimisation qui explorent l'espace de recherche en se déplaçant à
l'aveugle sont plus susceptibles de violer plusieurs contraintes simultanément dans de nombreuses
dimensions ; c'est le cas de l'\gls{PSO}. Les méthodes qui opèrent des mouvements sélectifs dans
chaque dimension, selon la violation de la contrainte et la valeur objectif de chaque vol, sont au
contraire plus efficaces ; c'est le cas de l'\gls{DE} et de l'\gls{GA} doté d'un opérateur de
croisement adapté, qui se sont avérés plus performants que l'\gls{PSO} sur le jeu de tests
considéré. Rappelons toutefois qu'il est parfois difficile d'ajuster les hyperparamètres des
algorithms stochastiques.

Ces résultats préliminaires indiquent que résoudre le problème de résolution de conflits dans un
espace de recherche continu est une alternative viable aux méthodes existantes. La modélisation
adoptée permet d'exprimer les man\oe uvres proposées comme une suite de points géographiques,
directement utilisables par les \gls{FMS}. Néanmoins, notre modèle n'est limité qu'aux man\oe uvres
latérales et devrait être enrichi de man\oe uvres verticales et en vitesse. Les incertitudes sur les
positions futures et sur les vitesses ne sont pas non plus considérées dans notre modèle simplifié.

\section{Optimal lateral maneuvers}
\label{sec:conflits-charibde}
De nombreux domaines de l'ingénierie font intervenir un invariant dans
leurs lois de commandes: "se déplacer à au moins un mètre du bord ", "conserver un niveau
de batterie supérieur à 50\%", etc. Une alternative à la résolution approchée décrite dans la
section précédente est de considérer la contrainte de séparation:
\begin{equation}
\quad S^2 \le \|\vec{p_i}(t) - \vec{p_j}(t)\|_2^2, \quad \forall t \in [0, T_f]
\end{equation}
comme une \gls{SIC} (Definition \ref{def:iuq}) et de résoudre le
problème de résolution de conflits grâce à un panel de techniques d'intervalles spécifiques.
Celles-ci sont décrites dans la suite de la section, et font intervenir un paramètre $p$,
correspondant ici au paramètre temporel $t$ de l'équation \ref{eq:contrainte-separation}.

\begin{definition}[Semi-infinite constraint]
Soit $c(x_1, \ldots, x_n, p)$ une fonction de $n$ variables réelles $(x_1, \ldots, x_n) \in (X_1,
\ldots, X_n)$ et d'un paramètre réel $p \in P$. On appelle \gls{SIC} la contrainte:
\begin{equation}
c(x_1, \ldots, x_n, p) \le 0, \quad \forall p \in P
\end{equation}
On note $\rho_c$ la relation définie par l'\gls{SIC} $c$:
\begin{equation}
\rho_c \eqdef \{(x_1, \ldots, x_n) \in X_1 \times \ldots \times X_n ~|~ c(x_1, \ldots, x_n, p) \le 0, \forall
p \in P \}
\end{equation}
\label{def:iuq}
\end{definition}

Un test de réfutation permettant de prouver qu'une boîte $\bm{X}$ ne contient aucune solution de 
$c$, c'est-à-dire que $\bm{X} \cap \rho_c = \varnothing$, est donné par:
\begin{equation}
\bm{X} \cap \rho_c = \varnothing \quad \Leftrightarrow \quad \exists p \in P, \quad
\exists (x_1, \ldots, x_n) \in \bm{X}, \quad c(x_1, \ldots, x_n, p) > 0
\label{eq:violation-sic}
\end{equation}

Dans cette section, nous étendons le modèle précédemment proposé, basé sur des man\oe uvres
rectilignes par morceaux, et proposons une résolution optimale des conflits certifiée par
Interval arithmetic~\cite{Vanaret2014}. Les méthodes par intervalles écartent la possibilité de détecter les
conflits entre deux trajectoires en calculant la distance minimale entre segments respectifs pendant
un même intervalle de temps. L'approche utilisée ici est l'utilisation d'une unique expression
analytique caractérisant la position d'un avion sur sa trajectoire à tout instant.

\subsection{Expression of the position}
On note (voir Figure \ref{fig:lateral-maneuver}):
\begin{itemize}
\item $\vec{u_1}$ the unitary vector along the initial trajectory ;
\item $\vec{u_2}$ the unitary vector along the deviation segment ;
\item $\vec{u_3}$ the unitary vector along the return segment ;
\item $T_1 = \frac{d}{v}$ the starting time of the maneuver ;
\item $T_2 = T_1 + \frac{l}{v}$ the starting time on the return segment ;
\item $T_3 = T_2 + \frac{l}{v}$ the time of return to the initial trajectory.
\end{itemize}

\begin{figure}[htbp]
\centering
\def\svgwidth{0.6\columnwidth}
\input{figures/trajectoire.pdf_tex}
\caption{Lateral maneuver}
\label{fig:lateral-maneuver}
\end{figure}

Let $v$ be the constant velocity norm of the aircraft. The velocity vector $\vec{v}(t)$ equals to
$\vec{v_1} = v \vec{u_1}$ on the time interval $[0, T_1]$, to $\vec{v_2} = v \vec{u_2}$ on
$[T_1, T_2]$, to $\vec{v_3} = v \vec{u_3}$ on $[T_2, T_3]$ and to $\vec{v_1}$ on $[T_3, T_f]$.
The velocity vector may thus be written at any time $t$ as a convex combination of the three velocities
$\vec{v_1}$, $\vec{v_2}$ and $\vec{v_3}$:
\begin{equation}
\begin{aligned}
\vec{v}(t) 	& = \left(1 - H(t-T_1) + H(t-T_3)\right) \vec{v_1} + \left(H(t-T_1) - H(t-T_2)\right)
\vec{v_2} \\
			& \quad + (H(t-T_2) - H(t-T_3)) \vec{v_3} \\
			& = \vec{v_1} + (\vec{v_2} - \vec{v_1}) H(t-T_1) +
			(\vec{v_3} - \vec{v_2}) H(t-T_2) + (\vec{v_1} - \vec{v_3}) H(t-T_3) \\
			& = v \left( \vec{u_1} + (\vec{u_2} - \vec{u_1}) H(t-T_1) +
			(\vec{u_3} - \vec{u_2}) H(t-T_2) + (\vec{u_1} - \vec{u_3}) H(t-T_3) \right)
\end{aligned}
\end{equation}
where $H: \mathbb{R} \rightarrow [0, 1]$ is the Heaviside step function:
\begin{equation}
\forall x \in \mathbb{R}, \quad H(x)=
\left\{
	\begin{matrix}
	0 			& \mathrm{si} & x < 0 \\
	1 			& \mathrm{si} & x \ge 0
	\end{matrix}
\right.
\end{equation}

Let $\vec{p_0}$ be the initial position of the aircraft. Its position at time $t$ is obtained
by integrating the velocity between 0 and $t$:
\begin{equation}
\begin{aligned}
\vec{p}(t) 	& = \int_0^t \vec{v}(u) du \\
			& = \vec{p_0} + v \left( \vec{u_1}t + (\vec{u_2}-\vec{u_1}) \max(0, t-T_1) +
(\vec{u_3}-\vec{u_2}) \max(0, t-T_2) \right. \\
			& \quad \left. + (\vec{u_1}-\vec{u_3}) \max(0, t-T_3) \right)
\end{aligned}
\end{equation}

En notant $\vec{d} = \begin{pmatrix} d_x \\ d_y \end{pmatrix}$ le vecteur directeur de la
trajectoire initiale (soit $\vec{d} = \vec{u_1}$) et
\begin{equation}
\beta = \begin{cases}
\arccos(d_x) 	& \text{if } d_y \ge 0 \\
-\arccos(d_x)	& \text{otherwise}
\end{cases}
\end{equation}
on obtient les vecteurs $\vec{u_3} - \vec{u_2}$, $\vec{u_2}$ et $\vec{u_3}$ par un raisonnement
trigonométrique:
\begin{align}
\vec{u_3} - \vec{u_2} = \begin{pmatrix} 2\sin(\alpha) d_y \\ -2\sin(\alpha) d_x \end{pmatrix} &
\qquad
\vec{u_2} = \begin{pmatrix} \cos(\alpha + \beta) \\ \sin(\alpha + \beta) \end{pmatrix} & \qquad
\vec{u_3} = \begin{pmatrix} \cos(\alpha - \beta) \\ \sin(\beta - \alpha) \end{pmatrix}
\end{align}

\subsection{Contraction strategies}
\label{sec:conflits-contracteur}
Dans cette section, nous détaillons les différentes techniques d'intervalles permettant de
contracter une boîte par rapport à une \gls{SIC}. Ces techniques incluent notamment la réduction du
domaine du paramètre et la contraction de la boîte après instanciation du paramètre. L'algorithm
\ref{algo:contracter-iuq} détaille l'implémentation du contracteur principal de Charibde spécifique
aux \gls{SIC}. Les briques qui le composent sont détaillées dans les paragraphes suivants.

\clearpage

\begin{algorithm}[htbp]
\caption{Contraction with respect to a semi-infinite constraint}
\label{algo:contracter-iuq}
\begin{algorithmic}
\Function{ContractSIC}{\inout{} $\bm{X}$: box, $g$: \gls{SIC}, \inout{} $P$: domain of parameter $p$}
\If{$P$ degenerate}
	\State \Call{Contract2B}{$\bm{X}, g, P$}
	\Comment Algorithm \ref{algo:contract-2b}
\Else
	\If{$g$ monotonic wrt $p$ over $P$}
		\State \Call{InstantiateParameter}{$\bm{X}, g, P$}
		\Comment equivalent constraint
		\State \Call{Contract2B}{$\bm{X}, g, P$}
		\Comment Algorithm \ref{algo:contract-2b}
	\Else
		\State \Call{InstantiateParameter}{$\bm{X}, g, P$}
		\Comment Algorithm \ref{algo:instantiate-parameter}
		\State \Call{Contract2B}{$\bm{X}, g, P$}
		\Comment Algorithm \ref{algo:contract-2b}
		\State \Call{ContractNegation}{$\bm{X}, g, P$}
		\Comment Algorithm \ref{algo:contract-negation}
		\State \Call{ShaveParameter}{$\bm{X}, g, P$}
		\Comment Algorithm \ref{algo:shave-parameter}
	\EndIf
\EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}

\subsubsection{2B contraction}
L'invocation d'un opérateur de cohérence partielle (par exemple 2B) sur la boîte $\bm{X}$ peut 
contracter les variables du problème, ainsi que le paramètre $p$. Une contraction sur $P$ indique 
que certaines valeurs du domaine sont incohérentes avec l'\gls{SIC}, auquel cas la boîte $\bm{X}$ 
est éliminée (algorithm \ref{algo:contract-2b}).

\begin{algorithm}[htbp]
\caption{2B contraction with respect to a semi-infinite constraint}
\label{algo:contract-2b}
\begin{algorithmic}
\Function{Contract2B}{\inout{} $\bm{X}$: box, $g$: \gls{SIC}, \inout{} $P$: domain of parameter $p$}
\State $P' \gets P$
\State $G_{\bm{X},P'} \gets $ \Call{HC4Revise}{$G(\bm{X}, P') \le 0$}
\If{$\bm{X} = \varnothing$ or $P' = \varnothing$ or $w(P') < w(P)$}
	\State constraint is violated
\ElsIf{$\overline{G_{\bm{X},P'}} \le 0$}
	\State constraint is satisfied
\EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}

\subsubsection{Instantiation of the parameter to a particular value}
L'\gls{SIC} $g$ doit être vérifiée quelle que soit la valeur du paramètre dans son domaine.
Contracter $g$ en ayant au préalable instancié $p$ à une valeur particulière $\hat{p}$ de son
domaine offre un pouvoir filtrant élevé et peut permettre d'éliminer la boîte si la contrainte
est violée pour cette valeur particulière (voir équation \ref{eq:violation-sic}).

Lorsque l'\gls{SIC} $g$ est monotone par rapport au paramètre $p$ sur $(\bm{X}, P)$, la valeur
optimale de $\hat{p}$ est une des bornes de $P$ ; il y a alors équivalence des
contraintes~\cite{Goldsztejn2009Efficient}. Lorsque $g$ est croissante (respectivement décroissante)
par rapport à $p$, la contrainte $G(\bm{X}, P) \le 0$ est équivalente à la contrainte $G(\bm{X},
\overline{P}) \le 0$ (respectivement $G(\bm{X}, \underline{P}) \le 0$).

Dans le cas contraire, on peut choisir arbitrairement le milieu de l'intervalle: $\hat{p} = m(P)$
(algorithm \ref{algo:instantiate-parameter}).

\begin{algorithm}[htbp]
\caption{Instantiation of the parameter}
\label{algo:instantiate-parameter}
\begin{algorithmic}
\Function{ContractWithInstantiatedParameter}{\inout{} $\bm{X}$: box, $g$: \gls{SIC}, \inout{} $P$: domain of parameter $p$}
\If{$g$ monotonic with respect to $p$ over $P$}
	\State $\hat{p} \gets$ appropriate bound of $P$
\Else
	\State $\hat{p} \gets m(P)$
\EndIf
\State \Call{HC4Revise}{$G(\bm{X}, \hat{p}) \le 0$}
\If{$\bm{X} = \varnothing$}
	\State $g$ is violated over $\bm{X}$
\EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}

\subsubsection{Contraction of the parameter's domain}
Lorsque la boîte courante $\bm{X}$ n'est pas réfutable par les tests précédents, contracter $\bm{X}$
par rapport à la \textit{négation de la contrainte} permet de réduire le domaine du paramètre en
éliminant des valeurs qui satisfont l'\gls{SIC}
initiale~\cite{Benhamou2000Universally,Goldsztejn2009Efficient}.

\begin{algorithm}[htbp]
\caption{Contraction of the parameter's domain}
\label{algo:contract-negation}
\begin{algorithmic}
\Function{ContractNegation}{\inout{} $\bm{X}$: box, $g$: \gls{SIC}, \inout{} $P$: domain of parameter $p$}
\State $\bm{X'} \gets \bm{X}$
\State $P' \gets P$
\State \Call{HC4Revise}{$G(\bm{X'}, P') > 0$}
\Comment contraction of $\bm{X'}$ and $P'$
\If{$\bm{X'} = \varnothing$}
	\State $g$ is satisfied over $(\bm{X}, \bm{P})$
\Else
	\State $P \gets P'$
\EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}

\subsubsection{Shaving of the parameter's domain}
The shaving strategy that inspired consistency operators $k$B and CID may be exploited to reduce
the parameter's domain~\cite{Collavizza1999Extending}. Evaluating the constraint on a slice $P_i \subset P$
decreases the overestimation induced by dependency, and improves the enclosure of the constraint
(Algorithm \ref{algo:shave-parameter}).

If $0 < G(\bm{X}, P_i)$, the \gls{SIC} is violated over the box $\bm{X}$ (see Equation \ref{eq:violation-sic}).
If $G(\bm{X}, P_i) \le 0$, it is not necessary to subsequently check feasibility on the slice $P_i$, and
the domain $P$ of the parameter $p$ is reduced to $P \setminus P_i$.

\begin{algorithm}[htb]
\caption{Shaving of the parameter's domain}
\label{algo:shave-parameter}
\begin{algorithmic}
\Function{ShaveParameter}{\inout{} $\bm{X}$: box, $g$: \gls{SIC}, \inout{} $P$: domain of parameter $p$, $s$: number of slices}
\State $P_\square \gets \varnothing$
\For{$i = \{1, \ldots, s\}$}
	\State $P_i \gets $ \Call{Slice}{$P, i, s$}
    
    \If{$g$ monotonic wrt $p$ over $P_i$}
		\State remplacer $P_i$ par une de ses bornes
		\Comment equivalent constraint
	\Else
		\State \Call{ContractWithInstantiatedParameter}{$\bm{X}, g, P_i$}
		\Comment Algorithm \ref{algo:instantiate-parameter}
	\EndIf
    
    
    \State \Call{Contracter2B}{$\bm{X}, g, P_i$}
	\If{$g$ is not violated over $(\bm{X}, P_i)$}
		\State $P_\square \gets \square(P', P_i)$
	\EndIf
\EndFor
\State $P \gets P_\square$
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{figure}[h!]
\centering
\def\svgwidth{0.8\columnwidth}
\input{figures/rognage.pdf_tex}
\caption{Shaving of the parameter's domain}
\label{fig:shaving-sip}
\end{figure}

La Figure \ref{fig:shaving-sip} illustre l'encadrement par Interval arithmetic d'une \gls{SIC} en fonction de
la valeur du paramètre $p$. Le domaine $P$ est découpé en $s$ bandelettes. L'évaluation de la
contrainte sur la première bandelette $P_1$ est négative, $P$ est donc réduit à $P \setminus P_1$.
La dernière bandelette $P_s$ est un intervalle indécidable car l'évaluation de la contrainte
contient 0. En
revanche, l'évaluation sur la bandelette $P_k$ est strictement positive, ce qui prouve que
l'\gls{SIC} n'est pas satisfaite pour toutes les valeurs du paramètre. La contrainte est donc violée
sur la boîte $(\bm{X}, P)$.

\subsubsection{Bisection of the parameter's domain}
\cite{Benhamou2000Universally,Goldsztejn2009Efficient} suggest to bisect the parameter's domain when
evaluating the constraint over a partition $\{P_1, P_2\}$ of the parameter's domain $P$ provides a satisfactory decrease in
the interval overestimation:
\begin{equation}
w(\square(C(\bm{X}, P_1), C(\bm{X}, P_2))) < \kappa \cdot w(C(\bm{X}, P))
\end{equation}
where $\kappa$ is a user-defined parameter. The constraint:
\begin{equation}
c(\bm{x}, p) \le 0, \quad \forall p \in P
\end{equation}
is then transformed into two distinct constraints:
\begin{equation}
c(\bm{x}, p_1) \le 0, \quad \forall p_1 \in P_1 \qquad \land \qquad
c(\bm{x}, p_2) \le 0, \quad \forall p_2 \in P_2
\end{equation}

\subsection{Test problems}
Les problèmes de test considérés sont trois instances à deux avions et trois instances à trois
avions, initialement en conflit. Les configurations à deux avions incluent:
\begin{itemize}
\item le face à face (Figure \ref{fig:initial-face-a-face}): les deux avions sont placés l'un
en face de l'autre, et volent l'un vers l'autre à la même vitesse (400 kts) ;
\item le dépassement (Figure \ref{fig:initial-depassement}): les deux avions se suivent à
distance sur la même trajectoire, l'avion de tête (volant à 400 kts) étant rattrapé par l'autre
appareil, plus rapide (480 kts) ;
\item le croisement (Figure \ref{fig:initial-croisement}): les trajectoires intiales des avions
se croisent perpendiculairement en début de trajectoires. Les avions volent à la même vitesse (400
kts).
\end{itemize}
Afin de réduire les symétries des trois problèmes, une contrainte de signe est ajoutée sur l'angle
de man\oe uvre d'un des deux avions.

\clearpage

\begin{figure}[htb]
\centering
\includegraphics[width=0.8\columnwidth]{expes/conflits/optimal/initial/face_a_face}
\caption{Configuration initiale en face à face}
\label{fig:initial-face-a-face}
\end{figure}

\begin{figure}[htb]
\centering
\includegraphics[width=0.8\columnwidth]{expes/conflits/optimal/initial/depassement}
\caption{Configuration initiale en dépassement}
\label{fig:initial-depassement}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.7\columnwidth]{expes/conflits/optimal/initial/croisement}
\caption{Configuration initiale en croisement}
\label{fig:initial-croisement}
\end{figure}

Les configurations à trois avions incluent:
\begin{itemize}
\item la configuration symétrique (Figure \ref{fig:initial-conflits3}): deux avions volent en
face à face, un troisième les croise perpendiculairement. Les avions volent à la même vitesse (400
kts) ;
\item la configuration bruitée (Figure \ref{fig:initial-conflits3-rand}): les avions sont placés
comme dans la configuration symétrique, et leurs caps sont légèrement bruités. Les avions volent à
la même vitesse (400 kts) ;
\item le rond-point (Figure \ref{fig:initial-conflits3-rp}): les trois avions sont disposés
régulièrement sur un cercle et convergent vers son centre à la même vitesse (400 kts).


\begin{figure}[htb]
\centering
\includegraphics[width=0.54\columnwidth]{expes/conflits/optimal/initial/conflits3}
\caption{Configuration initiale symétrique à trois avions}
\label{fig:initial-conflits3}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.59\columnwidth]{expes/conflits/optimal/initial/conflits3_rand}
\caption{Configuration initiale bruitée à trois avions}
\label{fig:initial-conflits3-rand}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.59\columnwidth]{expes/conflits/optimal/initial/conflits3_rp}
\caption{Configuration initiale en rond-point à trois avions}
\label{fig:initial-conflits3-rp}
\end{figure}
\end{itemize}

\subsection{Experimental results}
Nous présentons dans cette section les résultats optimaux certifiés par Charibde, pour une norme de
séparation de $S = 5 NM$. Le contracteur spécifique aux \gls{SIC} invoque les techniques présentées
dans la sous-section \ref{sec:conflits-contracteur}, en optant soit pour une stratégie de rognage,
soit pour une stratégie de bissection du domaine. Le contracteur 3BCID(20), hybridant les
algorithms de rognage 3B et CID, est utilisé pour l'intégralité des résultats expérimentaux.

\subsubsection{Conflicts between two aircraft}
Les trois instances à deux avions (6 variables) sont résolues avec les hyperparamètres du tableau
\ref{tab:conflits2-param}. Les variables de décision du problème ont pour domaine $(d_i, \alpha_i,
l_i) \in ([0, 100], [-\frac{\pi}{6}, \frac{\pi}{6}], [0, 100])$. Les résultats de Charibde sont
donnés dans le tableau \ref{tab:conflits2-stats}. Les solutions optimales obtenues sont présentées
respectivement dans les Figures
\ref{fig:solution-face-a-face} (face à face), \ref{fig:solution-croisement} (croisement) et
\ref{fig:solution-depassement} (dépassement).

\begin{table}[h!]
	\centering
	\caption{Conflits à deux avions: hyperparamètres de Charibde}
	\label{tab:conflits2-param}
	\begin{tabular}{|lc|}
	\hline
	Hyperparamètre 								& Valeur \\
	\hline
	$\varepsilon$ (précision) 					& $10^{-3}$ \\
	$\mathit{NP}$ (taille de la population) 	& 30 \\
	$W$ (facteur d'amplitude) 					& 0.7 \\
	$\mathit{CR}$ (taux de croisement) 		& 0.9 \\
	Bissection									& Largest \\
	Priorité									& MaxDist \\
	$\eta$ (ratio de point fixe)				& 0.8 \\
	Stratégie IUQ								& Rognage \\
	\hline
	\end{tabular}
\end{table}

\begin{table}[htb]
	\centering
	\caption{Conflits à deux avions: résultats de Charibde}
	\label{tab:conflits2-stats}
	\begin{tabular}{|lccc|}
	\hline
						& Face à face 	& Croisement 	& Dépassement \\
	\hline
	$\tilde{f}$			& 0.8420		& 0.9466		& 1.1762 \\
	Temps CPU (s) 		& 1.5 			& 0.6 			& 2.5 \\
	Bissections			& 28 			& 9 			& 39 \\
	Taille maximale de $\mathcal{Q}$ & 7 		& 5				& 7 \\
	Nombre d'évaluations de $F$ (\gls{IBC}) & 141976 & 64083 & 316833 \\
	Nombre d'évaluations de $\nabla F$ (\gls{IBC}) & 74 & 28 & 102 \\
	Nombre d'évaluations de $f$ (\gls{DE}) & 9057 & 4517 & 6027 \\
	Nombre d'évaluations de $F$ (\gls{DE}) & 71 & 30 & 49 \\
	\hline
	\end{tabular}
\end{table}

Dans les man\oe uvres optimales obtenues par Charibde, un seul des deux avions est dévié. Ceci
résulte de l'utilisation d'une somme dans la fonction objectif. Un coût basé sur le maximum des
déviations individuelles fournirait en revanche une solution plus "équitable", dans
laquelle tous les avions sont man\oe uvrés, avec des déviations plus faibles.

\begin{figure}[h!]
\centering
\includegraphics[width=0.75\columnwidth]{expes/conflits/optimal/solutions/face_a_face}
\caption{Solution optimale à deux avions en face à face}
\label{fig:solution-face-a-face}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.7\columnwidth]{expes/conflits/optimal/solutions/croisement}
\caption{Solution optimale à deux avions en croisement}
\label{fig:solution-croisement}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.75\columnwidth]{expes/conflits/optimal/solutions/depassement}
\caption{Solution optimale à deux avions en dépassement}
\label{fig:solution-depassement}
\end{figure}

\subsubsection{Conflicts between three aircraft}
Les trois instances à trois avions (9 variables) sont résolues avec les hyperparamètres du tableau
\ref{tab:conflits3-param}. Les variables de décision du problème ont pour domaine $(d_i, \alpha_i,
l_i) \in ([0, 40], [-\frac{\pi}{6}, \frac{\pi}{6}], [0, 40])$. Les résultats de Charibde sont
donnés dans le tableau \ref{tab:conflits3-stats}.

Différentes stratégies de réduction du domaine du
paramètre ont été utilisées: les résultats pour les configurations symétrique et bruitée ont été
obtenus avec un opérateur basé sur la bissection du paramètre, et les résultats pour la
configuration en rond-point ont été obtenus en utilisant un contracteur basé sur le rognage.
Les solutions optimales obtenues sont présentées respectivement dans les Figures
\ref{fig:solution-symetrique} (configuration symétrique), \ref{fig:solution-bruitee} (configuration
bruitée) et \ref{fig:solution-rp} (configuration en rond-point).

La configuration symétrique est résolue en 24 minutes. Les symétries du problème, non exploitées
ici, ralentissent l'exploration exhaustive de l'espace de recherche. Lorsque les symétries sont
brisées, la configuration bruitée est résolue en 4 minutes. La configuration en rond-point
apparaît comme un problème extrêmement difficile à résoudre, de nombreuses solutions équivalentes
devant être éliminées: la solution optimale est obtenue après 11.5 heures. Ces résultats
préliminaires, guère satisfaisants, reposent sur une modélisation dont la fonction objectif n'est
pas suffisamment discriminante. 

\begin{table}[h!]
	\centering
	\caption{Conflits à trois avions: hyperparamètres de Charibde}
	\label{tab:conflits3-param}
	\begin{tabular}{|lccc|}
	\hline
	Hyperparamètre 							& Symétrique 	& Bruitée 		& Rond-point \\
	\hline
	$\varepsilon$ (précision) 				& $10^{-1}$ 	& $10^{-1}$		& $10^{-1}$ \\
	$\mathit{NP}$ (taille de la population) & 30 			& 50			& 30 \\
	$W$ (facteur d'amplitude) 				& 0.7 			& 0.7 			& 0.7 \\
	$\mathit{CR}$ (taux de croisement) 		& 0.9 			& 0.9 			& 0.9 \\
	Bissection								& Largest 		& Largest 		& Largest \\
	Priorité								& MaxDist 		& MaxDist 		& MaxDist \\
	$\eta$ (ratio de point fixe)			& 0.8 			& 0.8 			& 0.8\\
	Stratégie IUQ							& Bissection ($\kappa = 0.8$) 	& Bissection ($\kappa =
0.8$)	& Rognage \\
	\hline
	\end{tabular}
\end{table}

\begin{table}[h!]
	\centering
	\caption{Conflits à trois avions: résultats de Charibde}
	\label{tab:conflits3-stats}
	\begin{tabular}{|lccc|}
	\hline
		 									& Symétrique 	& Bruitée 	& Rond-point \\
	\hline
	$\tilde{f}$								& 1.8453	 	& 2.0420	& 3.2335 \\
	Temps CPU (s) 							& 1432 			& 242 		& 41340 \\
	Bissections								& 31473 		& 1330 		& 129743 \\
	Taille maximale de $\mathcal{Q}$		& 46 			& 13 		& 19 \\
	Nombre d'évaluations de $F$ (\gls{IBC}) & 132163387 	& 15347706 	& 2425978874 \\
	Nombre d'évaluations de $\nabla F$ (\gls{IBC}) & 74080 	& 2969 		& 287221 \\
	Nombre d'évaluations de $f$ (\gls{DE}) 	& 42205811 		& 811090 	& 36964505 \\
	Nombre d'évaluations de $F$ (\gls{DE}) 	& 399 			& 286 		& 6057 \\
	\hline
	\end{tabular}
\end{table}

\begin{figure}[h!]
\centering
\includegraphics[width=0.55\columnwidth]{expes/conflits/optimal/solutions/conflits3}
\caption{Solution optimale à trois avions en configuration symétrique}
\label{fig:solution-symetrique}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.55\columnwidth]{expes/conflits/optimal/solutions/conflits3_rand}
\caption{Solution optimale à trois avions en configuration bruitée}
\label{fig:solution-bruitee}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.55\columnwidth]{expes/conflits/optimal/solutions/conflits3_rp}
\caption{Solution optimale à trois avions en configuration rond-point}
\label{fig:solution-rp}
\end{figure}

\clearpage

\section{Perspectives}
La vitesse d'un appareil en vol est sujette à des incertitudes en raison du manque de fiabilité des
mesures radar au sol. La connaissance de la position future de l'appareil se dégrade donc avec le
temps, jusqu'à ce que la mesure radar suivante permette de rafraîchir l'incertitude sur la position.
Par exemple, \cite{Durand1996} résout les conflits en prenant en compte les incertitudes sur la
vitesse: l'augmentation de la taille de l'espace de recherche est gérée par les \gls{EA}.

Les techniques basées sur le calcul par intervalles sont intrinsèquement capables de résoudre des
problèmes d'optimisation lorsque certains paramètres sont incertains. La vitesse incertaine d'un
avion peut s'écrire sous la forme d'un intervalle:
\begin{equation}
v_{int} = [1 - p, 1 + p] v_{nom}
\end{equation}
où $v_{nom}$ est la vitesse nominale d'un avion en croisière (de l'ordre de 400 n\oe uds) et $p =
5\%$. Une perspective intéressante serait d'étendre notre modèle en intégrant la vitesse comme
deuxième paramètre et de résoudre le problème sous contraintes d'\gls{SIC} avec les techniques de
contraction
décrites précédemment.


==> garde.tex <==
%~ \begin{center}
%~ 
%~ \vspace*{5cm}
%~ 
%~ {\bf En vue de l'obtention du}
%~ 
%~ \medskip
%~ 
%~ {\Large {\bf DOCTORAT DE L'UNIVERSITÉ DE TOULOUSE}}
%~ 
%~ \bigskip
%~ 
%~ {\bf Délivré par :}
%~ 
%~ \smallskip
%~ 
%~ {\large Institut National Polytechnique de Toulouse (INP Toulouse)}
%~ 
%~ \medskip
%~ 
%~ {\bf Discipline ou spécialité :}
%~ 
%~ \smallskip
%~ 
%~ {\large Informatique et Télécommunications}
%~ 
%~ \smallskip
%~ 
%~ \rule{\linewidth}{1pt}
%~ 
%~ \medskip
%~ 
%~ {\bf Présentée et soutenue par :}
%~ 
%~ \medskip
%~ 
%~ Charlie Vanaret
%~ 
%~ \medskip
%~ 
%~ {\bf le:} xxxxxx 2014
%~ 
%~ \medskip
%~ 
%~ {\large {\bf Titre :}}
%~ 
%~ \medskip
%~ 
%~ {\Large Hybridation de Branch and Bound par intervalles et de stratégies
%~ évolutionnaires pour l'optimisation de problèmes difficiles}
%~ 
%~ \rule{\linewidth}{1pt}
%~ 
%~ \bigskip
%~ 
%~ {\bf École doctorale :}
%~ 
%~ Mathématiques Informatique Télécommunications (MITT)
%~ 
%~ \smallskip
%~ 
%~ {\bf Unité de recherche :}
%~ 
%~ IRIT \--- Algorithmes Parallèles et Optimisation (APO)
%~ 
%~ \smallskip
%~ 
%~ {\bf Directeur de thèse :}
%~ 
%~ Nicolas Durand
%~ 
%~ \bigskip
%~ 
%~ {\bf Jury :}
%~ 
%~ \smallskip
%~ 
%~ \begin{tabular}{llr}
%~ Dr Jean-Baptiste Gotteland & ENAC & Examinateur\\
%~ Dr Nicolas Durand & ENAC \hspace*{2cm}& Directeur de thèse\\
%~ Pr Éric Féron & Georgia Institute of Technology & Examinateur\\
%~ Pr Pierre Flener & Uppsala University & Rapporteur\\
%~ Pr Jin-Kao Hao & Université d'Angers & Rapporteur\\
%~ Dr Xavier Prats & Universitat Politècnica de Catalunya & Examinateur
%~ \end{tabular}
%~ 
%~ \end{center}

\AddToShipoutPicture*{\put(0,0){\includegraphics{figures/couverture_vierge}}}
\thispagestyle{empty}

